Content Adaptive Optimization for Neural Image Compression

The field of neural image compression has witnessed exciting progress as recently proposed architectures already surpass the established transform coding based approaches. While, so far, research has mainly focused on architecture and model improvements, in this work we explore content adaptive optimization. To this end, we introduce an iterative procedure which adapts the latent representation to the specific content we wish to compress while keeping the parameters of the network and the predictive model fixed. Our experiments show that this allows for an overall increase in rate-distortion performance, independently of the specific architecture used. Furthermore, we also evaluate this strategy in the context of adapting a pretrained network to other content that is different in visual appearance or resolution. Here, our experiments show that our adaptation strategy can largely close the gap as compared to models specifically trained for the given content while having the benefit that no additional data in the form of model parameter updates has to be transmitted.

==> sections/figures.tex <==
\onecolumn 

\begin{figure}[]
	\includegraphics[width=\linewidth]{Tecnick_avg_curve_simple.pdf}
	\caption{Each point
		on the RD curves is calculated by averaging over the PSNR and bit rate values for the 100 Tecnick
		images for a single Q value (for standard codecs) or λ (for learned methods). Each Tecnick image
		has resolution 1200x1200. }
	\label{fig:simple}	
\end{figure}

\begin{figure}[]
	\includegraphics[width=\linewidth]{Tecnick_avg_curve_gmm.pdf}
	\caption{Each point
		on the RD curves is calculated by averaging over the PSNR and bit rate values for the 100 Tecnick
		images for a single Q value (for standard codecs) or λ (for learned methods). Each Tecnick image
		has resolution 1200x1200. }
	\label{fig:gmm}
\end{figure}

\twocolumn

==> sections/luciddreams-plots.tex <==
%-----------------------------------------------------
% General Plot Style Settings
%-----------------------------------------------------
\pgfplotsset{compat=1.14}
\pgfplotsset{grid style={color=black!15, },} % dashed
\pgfplotsset{every axis x grid/.style={draw opacity=0}}
\pgfplotsset{minor grid style={dashed,red}}
%\pgfplotsset{major grid style={dotted,green!50!black}}

\pgfplotsset{
	axis x line=bottom,
	axis y line=left,
	axis line style={draw=none},
	tick style={draw=none},
	grid,
	xmin=0, xmax=1,
	xlabel=Rate (bpp),
	legend style={at={(0.96,0.04)},anchor=south east},
	legend cell align={left},
	label style={font=\footnotesize},
	legend style={font=\tiny},
	%legend style={draw=none},
	legend style={draw=gray},
	tick label style={font=\footnotesize},
	width=0.725\columnwidth
}
\pgfplotsset{
	every axis plot/.append style={line width=1pt, cap=round, smooth},
	%	every axis plot post/.append style={
	%		every mark/.append style={line width=1.6pt,draw=green,fill=red}
	%	}
}

%--------------------------------------
% Some colors
%--------------------------------------

\definecolor{myBlue}{RGB}{41,77,165}
\definecolor{myBlueLight}{RGB}{164,185,226}
\definecolor{myOrange}{RGB}{231,116,46 }
\definecolor{myOrangeLight}{RGB}{239,177,105}
\definecolor{myGreen}{RGB}{78,145,41}
\definecolor{myGreenLight}{RGB}{160,219,207}
\definecolor{myRed}{RGB}{181,45,38}
\definecolor{myRedLight}{RGB}{233,138,133}
\definecolor{myMagenta}{RGB}{233,0,233}

%\newcommand{\bpg}{myBlue}
%\newcommand{\jpg}{myRedLight}
\newcommand{\lucid}{myOrange}
%\newcommand{\webp}{myGreen}
%\newcommand{\full}{myMagenta}

\begin{figure}[t]
	\hspace{-0.2cm}
	\begin{tikzpicture}[scale=1.45]
	\begin{axis}[ylabel=Distortion (PSNR),ymin=38, ymax=45,xmin=0.15, xmax=0.69,ytick={29, 31,...,45}, legend style={at={(0.4,.95)},anchor=north east,nodes={scale=0.6, transform shape}, row sep=0.0pt} ]
	\addplot[draw=\full, dashed, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/LucidDreams_HD/full_coco.csv};
	\addlegendentry{full-coco}
	\addplot[draw=\full, dotted, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/LucidDreams_HD/full_coco+proba.csv};
	\addlegendentry{full-coco+proba }
	\addplot[draw=\full, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/LucidDreams_HD/full_coco+adapt.csv};
	\addlegendentry{full-coco + adapt}
	\addplot[draw=\lucid, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/LucidDreams_HD/full_luciddreams.csv};
	\addlegendentry{full-lucid}
		\addplot[draw=\bpg, line width=0.25pt] table[x=bpp, y=psnr, col sep=comma] {evaluation/LucidDreams_HD/bpg444.csv};
	\addlegendentry{BPG}
	%	\addplot[draw=\jpg, line width=0.5pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Tecnick/jpeg.csv};
	%	\addlegendentry{JPEG}
	\addplot[draw=\webp, line width=0.25pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/LucidDreams_HD/webp.csv};
	\addlegendentry{Webp}
	\end{axis}
	\end{tikzpicture}
	\vspace{-0.3cm}
	\caption{\textbf{Evaluation Lucid dreams} ...}
	\label{fig:lucid_dreams}
\end{figure}



==> sections/meridian-plots.tex <==
%-----------------------------------------------------
% General Plot Style Settings
%-----------------------------------------------------
\pgfplotsset{compat=1.14}
\pgfplotsset{grid style={color=black!15, },} % dashed
\pgfplotsset{every axis x grid/.style={draw opacity=0}}
\pgfplotsset{minor grid style={dashed,red}}
%\pgfplotsset{major grid style={dotted,green!50!black}}

\pgfplotsset{
	axis x line=bottom,
	axis y line=left,
	axis line style={draw=none},
	tick style={draw=none},
	grid,
	xmin=0, xmax=1,
	xlabel=Rate (bpp),
	legend style={at={(0.96,0.04)},anchor=south east},
	legend cell align={left},
	label style={font=\footnotesize},
	legend style={font=\tiny},
	%legend style={draw=none},
	legend style={draw=gray},
	tick label style={font=\footnotesize},
	width=0.725\columnwidth
}
\pgfplotsset{
	every axis plot/.append style={line width=1pt, cap=round, smooth},
	%	every axis plot post/.append style={
	%		every mark/.append style={line width=1.6pt,draw=green,fill=red}
	%	}
}

%--------------------------------------
% Some colors
%--------------------------------------

\definecolor{myBlue}{RGB}{41,77,165}
\definecolor{myBlueLight}{RGB}{164,185,226}
\definecolor{myOrange}{RGB}{231,116,46 }
\definecolor{myOrangeLight}{RGB}{239,177,105}
\definecolor{myGreen}{RGB}{78,145,41}
\definecolor{myGreenLight}{RGB}{160,219,207}
\definecolor{myRed}{RGB}{181,45,38}
\definecolor{myRedLight}{RGB}{233,138,133}
\definecolor{myMagenta}{RGB}{233,0,233}

%\newcommand{\bpg}{myBlue}
%\newcommand{\jpg}{myRedLight}
\newcommand{\meridian}{myOrange}
%\newcommand{\webp}{myGreen}
%\newcommand{\full}{myMagenta}

\begin{figure}[t]
	\begin{tikzpicture}[scale=1.45]
	\begin{axis}[ylabel=Distortion (PSNR),ymin=40, ymax=47,xmin=0.05, xmax=0.45,ytick={29, 31,...,47}, legend style={at={(0.4,.95)},anchor=north east,nodes={scale=0.6, transform shape}, row sep=0.0pt} ]
	\addplot[draw=\full, dashed, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Meridian_HD/full_coco.csv};
	\addlegendentry{full-coco}
	\addplot[draw=\full, dotted, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Meridian_HD/full_coco+proba.csv};
	\addlegendentry{full-coco+proba }
	\addplot[draw=\full, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Meridian_HD/full_coco+adapt.csv};
	\addlegendentry{full-coco + adapt}
	\addplot[draw=\meridian, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Meridian_HD/full_meridian.csv};
	\addlegendentry{full-Meridian}
		\addplot[draw=\bpg, line width=0.25pt] table[x=bpp, y=psnr, col sep=comma] {evaluation/Meridian_HD/bpg444.csv};
	\addlegendentry{BPG}
	%	\addplot[draw=\jpg, line width=0.5pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Tecnick/jpeg.csv};
	%	\addlegendentry{JPEG}
	\addplot[draw=\webp, line width=0.25pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Meridian_HD/webp.csv};
	\addlegendentry{Webp}
	\end{axis}
	\end{tikzpicture}
	\vspace{-0.3cm}
	\caption{\textbf{Evaluation Meridian} ...}
	\label{fig:meridian}
\end{figure}



==> sections/netflix4k-plots.tex <==
%-----------------------------------------------------
% General Plot Style Settings
%-----------------------------------------------------
\pgfplotsset{compat=1.14}
\pgfplotsset{grid style={color=black!15, },} % dashed
\pgfplotsset{every axis x grid/.style={draw opacity=0}}
\pgfplotsset{minor grid style={dashed,red}}
%\pgfplotsset{major grid style={dotted,green!50!black}}

\pgfplotsset{
	axis x line=bottom,
	axis y line=left,
	axis line style={draw=none},
	tick style={draw=none},
	grid,
	xmin=0, xmax=1,
	xlabel=Rate (bpp),
	legend style={at={(0.96,0.04)},anchor=south east},
	legend cell align={left},
	label style={font=\footnotesize},
	legend style={font=\tiny},
	%legend style={draw=none},
	legend style={draw=gray},
	tick label style={font=\footnotesize},
	width=0.725\columnwidth
}
\pgfplotsset{
	every axis plot/.append style={line width=1pt, cap=round, smooth},
	%	every axis plot post/.append style={
	%		every mark/.append style={line width=1.6pt,draw=green,fill=red}
	%	}
}

%--------------------------------------
% Some colors
%--------------------------------------

\definecolor{myBlue}{RGB}{41,77,165}
\definecolor{myBlueLight}{RGB}{164,185,226}
\definecolor{myOrange}{RGB}{231,116,46 }
\definecolor{myOrangeLight}{RGB}{239,177,105}
\definecolor{myGreen}{RGB}{78,145,41}
\definecolor{myGreenLight}{RGB}{160,219,207}
\definecolor{myRed}{RGB}{181,45,38}
\definecolor{myRedLight}{RGB}{233,138,133}
\definecolor{myMagenta}{RGB}{233,0,233}

%\newcommand{\bpg}{myBlue}
%\newcommand{\jpg}{myRedLight}
\newcommand{\netflixhd}{myGreen}
\newcommand{\netflixFOURK}{myRed}
%\newcommand{\webp}{myGreen}
%\newcommand{\full}{myMagenta}

\begin{figure}[t]
	\begin{tikzpicture}[scale=1.45]
	\begin{axis}[ylabel=Distortion (PSNR),ymin=37, ymax=42,xmin=0.1, xmax=0.7,ytick={29, 31,...,47}, legend style={at={(0.95,.55)},anchor=north east,nodes={scale=0.65, transform shape}, row sep=0.0pt} ]
	%------------ COCO
	\addplot[draw=\full, dashed, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Netflix_4k/full_coco.csv};
	\addlegendentry{full-coco}
	\addplot[draw=\full, dotted, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Netflix_4k/full_coco+proba.csv};
	\addlegendentry{full-coco+proba }
	\addplot[draw=\full, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Netflix_4k/full_coco+adapt.csv};
	\addlegendentry{full-coco + adapt}
	%------------ netflixHD
	\addplot[draw=\netflixhd, dashed, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Netflix_4k/full_netflixHD.csv};
	\addlegendentry{full-NetflixHD}
	\addplot[draw=\netflixhd, dotted, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Netflix_4k/full_netflixHD+proba.csv};
	\addlegendentry{full-NetflixHD + proba }
	\addplot[draw=\netflixhd, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Netflix_4k/full_netflixHD+adapt.csv};
	\addlegendentry{full-NetflixHD + adapt}
	%------------ Netflix 4k
	\addplot[draw=\netflixFOURK, line width=0.5pt, mark=o, mark size=0.75pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Netflix_4k/full_netflix4k.csv};
	\addlegendentry{full-Meridian}
%		\addplot[draw=\bpg, line width=0.25pt] table[x=bpp, y=psnr, col sep=comma] {evaluation/Netflix_4k/bpg444.csv};
%	\addlegendentry{BPG}
%	%	\addplot[draw=\jpg, line width=0.5pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Tecnick/jpeg.csv};
%	%	\addlegendentry{JPEG}
%	\addplot[draw=\webp, line width=0.25pt] table [x=bpp, y=psnr, col sep=comma] {evaluation/Netflix_4k/webp.csv};
%	\addlegendentry{Webp}
	\end{axis}
	\end{tikzpicture}
	\vspace{-0.3cm}
	\caption{\textbf{Evaluation Netflix 4k} ...}
	\label{fig:netflix4k}
\end{figure}


